A Barrier Certificate-based Simplex Architecture for Systems with Approximate and Hybrid Dynamics

We present Barrier-based Simplex (Bb-Simplex), a new, provably correct design for runtime assurance of continuous dynamical systems. Bb-Simplex is centered around the Simplex control architecture, which consists of a high-performance advanced controller that is not guaranteed to maintain safety of the plant, a verified-safe baseline controller, and a decision module that switches control of the plant between the two controllers to ensure safety without sacrificing performance. In Bb-Simplex, Barrier certificates are used to prove that the baseline controller ensures safety. Furthermore, Bb-Simplex features a new automated method for deriving, from the barrier certificate, the conditions for switching between the controllers. Our method is based on the Taylor expansion of the barrier certificate and yields computationally inexpensive switching conditions. We also propose extensions to Bb-Simplex to enable its use in hybrid systems, which have multiple modes each with its own dynamics, and to support its use when only approximate dynamics (not exact dynamics) are available, for both continuous-time and hybrid dynamical systems. We consider significant applications of Bb-Simplex to microgrids featuring advanced controllers in the form of neural networks trained using reinforcement learning. These microgrids are modeled in RTDS, an industry-standard high-fidelity, real-time power systems simulator. Our results demonstrate that Bb-Simplex can automatically derive switching conditions for complex continuous-time and hybrid systems, the switching conditions are not overly conservative, and Bb-Simplex ensures safety even in the presence of adversarial attacks on the neural controller when only approximate dynamics (with an error bound) are available.

==> BC.tex <==
\subsection{Droop Controller as Baseline Controller}

We use a traditional droop controller as the baseline controller; see Fig.~\ref{fig:archi}. Using the methodology described below, we derive a Barrier Certificate (BaC) to establish proof of the BC's safety. This methodology is general enough to be applied to any type of controller.
\shortonly{
The dynamic model for a voltage droop controller for an inverter in an MG has the form $\dot{v}=v^*-v+\lambda_q(Q^*-Q)$, where $v^*,v,Q^*,Q$ are voltage reference, voltage, reactive power reference and reactive power of inverter, respectively, and $\lambda_q$ is the controller's droop coefficient. Detailed dynamic models for an MG with multiple inverters connected by transmission lines and with droop controllers for frequency and voltage are given in~\cite{LypStability,Kundu2019}.
}

Our\
methodology for computing switching conditions (see \journal{Section}\thesis{Chapter}~\ref{sec:DM}) requires a BaC, but is independent of how the BaC is obtained.
Currently we derive a Lyapunov function $V$ for the system using the expanding interior-point algorithm in~\cite{LypStability}, and then use the SOS-based algorithm in~\cite{permissiveBC,Kundu2019} to obtain a  BaC from the Lyapunov function. Note that the largest super-level set of a Lyapunov function within a safety region is a BaC. The algorithm in~\cite{permissiveBC,Kundu2019} computes a larger BaC by starting with that sub-level set and then expanding it, by allowing it to take shapes other than that of a sub-level set of the Lyapunov function. \fullonly{Fig.~\ref{fig:bac_plot} shows this process of incrementally expanding the Lyapunov function to obtain the BaC. }SOS-based algorithms apply only to polynomial dynamics, so we first recast droop controller dynamics to be polynomial using a DQ0 transformation \cite{dq0} to AC waveforms. This transformation is exact; i.e., it does not introduce any approximation error.  
\fullonly{
Other possible approaches to obtain polynomial dynamics are Taylor approximation~\cite{Kundu2019} and the recasting techniques in~\cite{LypStability}. 
}

Our methodology for deriving safety guarantees for the BC is as follows:
(1)~Obtain analytical dynamics for the plant + BC.
(2)~Convert non-polynomial dynamics to polynomial.
(3)~Compute a Lyapunov function for plant + BC using SOSTOOLS.
(4)~From the Lyapunov function, compute the BaC for plant + BC.
Steps~3 and~4 involve a search of Lyapunov functions and BaCs of various degrees by choosing different candidate polynomials and parameters of SOS problem.

In our experimental evaluation (\journal{Section}\thesis{Chapter}~\ref{sec:EE}), we used this methodology to obtain BaCs for BCs in the form of droop controllers for voltage regulation, in the context of MGs containing up to three DERs of different types. Note that battery DERs operate in two distinct modes, charging and discharging, resulting in a hybrid system model with different dynamics in different modes.  For now, we consider only runs in which the battery remains in the same mode for the duration of the run. Extending our framework to hybrid systems is future work.

